ForestNet: Classifying Drivers of Deforestation in Indonesia using Deep Learning on Satellite Imagery

Characterizing the processes leading to deforestation is critical to the development and implementation of targeted forest conservation and management policies. In this work, we develop a deep learning model called ForestNet to classify the drivers of primary forest loss in Indonesia, a country with one of the highest deforestation rates in the world. Using satellite imagery, ForestNet identifies the direct drivers of deforestation in forest loss patches of any size. We curate a dataset of Landsat 8 satellite images of known forest loss events paired with driver annotations from expert interpreters. We use the dataset to train and validate the models and demonstrate that ForestNet substantially outperforms other standard driver classification approaches. In order to support future research on automated approaches to deforestation driver classification, the dataset curated in this study is publicly available at https://stanfordmlgroup.github.io/projects/forestnet .

==> figures/figure1.tex <==
\begin{figure*}[ht!]
  \centering
    \begin{tabular}{cccc}
    \includegraphics[width=0.2\textwidth]{images/DriverExample1.png} & \includegraphics[width=0.2\textwidth]{images/DriverExample1.png} & \includegraphics[width=0.2\textwidth]{images/DriverExample1.png} & \includegraphics[width=0.2\textwidth]{images/DriverExample1.png}\\
    Plantation & Smallholder Agriculture & Grassland/shrubland & Mining \\
    \includegraphics[width=0.2\textwidth]{images/DriverExample1.png} & \includegraphics[width=0.2\textwidth]{images/DriverExample1.png} & \includegraphics[width=0.2\textwidth]{images/DriverExample1.png} & \includegraphics[width=0.2\textwidth]{images/DriverExample1.png}\\
    Fish Pond & Logging & Secondary Forest & Other
    \end{tabular}
  \caption{Characteristic examples of satellite imagery for each of the forest loss driver categories. Forest loss regions are overlaid here for demonstration but are not overlaid on the images when input to the models.}
  \label{fig:visual-comparison}
\end{figure*}

==> figures/figure_map.tex <==
% https://docs.google.com/drawings/d/16dyficY1e4vLvud4tSZrw_UeI5EbEWif7prOOKstTV4/edit?usp=sharing

\begin{figure*}[ht!]
  \centering
  \includegraphics[scale=0.25]{images/MapExample.png}
  \caption{
    Predicted major driver of deforestation in Indonesia, year 2018 (placeholder for now)
    \hao{One of our highlight plot is the map we made. I am thinking whether we want to have one of those maps appearing in the first page}
  }
  \label{fig:map}
\end{figure*}

